Differentially Private Algorithms for 2020 Census Detailed DHC Race \& Ethnicity

This article describes a proposed differentially private (DP) algorithms that the US Census Bureau is considering to release the Detailed Demographic and Housing Characteristics (DHC) Race & Ethnicity tabulations as part of the 2020 Census. The tabulations contain statistics (counts) of demographic and housing characteristics of the entire population of the US crossed with detailed races and tribes at varying levels of geography. We describe two differentially private algorithmic strategies, one based on adding noise drawn from a two-sided Geometric distribution that satisfies "pure"-DP, and another based on adding noise from a Discrete Gaussian distribution that satisfied a well studied variant of differential privacy, called Zero Concentrated Differential Privacy (zCDP). We analytically estimate the privacy loss parameters ensured by the two algorithms for comparable levels of error introduced in the statistics.

==> results.tex <==
\subsection{Results \& Discussion}
\begin{table}
  \centering
  \begin{tabular}{r l l l l}
    \toprule
    \textbf{Base Mechanism} & \multicolumn{2}{c}{Geometric} & \multicolumn{2}{c}{Discrete Gaussian} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    \textbf{Analysis} & Pure DP & RDP & zCDP (analytical) & zCDP (experimental) \\
    \midrule
    \textbf{$(\epsilon, 10^{-10})$ privacy loss} & 15.3 ($\delta = 0$) & 13.2 & 12.8 & 12.2 \\
    \bottomrule
  \end{tabular}
  \caption{The approximate differential privacy loss of the SafeTab[Geometric] and SafeTab[Discrete Gaussian] algorithm for various analyses. For all but the Pure DP analysis, $\delta=10^{-10}$. For the Pure DP analysis, $\delta=0$.}
  \label{tab:privacy-loss-results}
\end{table}
\paragraph{Privacy losses of Geometric vs Discrete Gaussian:}
Results appear in Table~\ref{tab:privacy-loss-results}. We observe the following key findings: 
\begin{itemize}
    \item The pure DP privacy loss of SafeTab[Geometric] is bounded by $\epsilon=15.3$. This is smaller than the $\epsilon=18$ that was analyzed by the Census POP team using the SafeTEx analysis tool. The lower privacy loss is due to two reasons: 
    \begin{enumerate}
        \item  The original SafeTEx analysis was done with a target MOE of 5.6 for Nation and State detailed population groups. We also updated the MOE to 6 since noise is integral and therefore it makes sense to use an integral MOE. 
        \item The original SafeTEx analysis was done assuming SafeTab used the base Laplace mechanism rather than the base geometric mechanism.
        The tail probability of the Geometric distribution are tighter than those of the Laplace distribution at integer points. This results in a smaller privacy loss.
    \end{enumerate}
    \item As expected SafeTab[Geometric] permits a smaller privacy loss ($\epsilon$) under approximate DP with ($\delta = 10^{-10}$). We are able to achieve this by analyzing SafeTab[Geometric] under R\'enyi DP. 
    \item We observe that the privacy loss of SafeTab[Discrete Gaussian] is smaller than that of SafeTab[Geometric] (when $\delta=10^{-10}$). The improvement in privacy loss is small (3\% for the analytical bound and 7\% for the experimental bound). 
\end{itemize}



\begin{table}[t]
  \centering
  \begin{tabular}{ c l l l l}
    \toprule  
    MOE for (Nation, Detailed) & \multicolumn{2}{c}{Geometric} & \multicolumn{2}{c}{Discrete Gaussian} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    and (State, Detailed) & Pure DP & RDP & zCDP (analytical) & zCDP (experimental) \\
    \midrule
     5 & 16.7 ($\delta = 0$) & 14.6 & 15.0 & 14.3 \\
     6 & 15.3 ($\delta = 0$) & 13.2 & 12.8 & 12.2 \\
     7 & 14.2 ($\delta = 0$) & 12.1 & 11.3 & 10.7 \\
     8 & 13.4 ($\delta = 0$) & 11.3 & 10.2 & 9.7 \\
     9 & 12.7 ($\delta = 0$) & 10.7 & 9.5 & 9.0 \\
     10 & 12.2 ($\delta = 0$) & 10.2 & 8.9 & 8.4  \\
     11 & 11.7 ($\delta = 0$) & 9.7 & 8.4 & 8.0 \\
    \bottomrule
  \end{tabular}
  \caption{The approximate differential privacy loss of the SafeTab[Geometric] and SafeTab[Discrete Gaussian] algorithm when $\delta=10^{-10}$ for alternate MOE values for the (Nation, Detailed) and (State, Detailed) population group levels. MOEs for all other population group levels are fixed as in Table~\ref{tab:moe-targets}.}
  \label{tab:alternate-moes}
\end{table}

\paragraph{Granularity of Statistics under Geometric vs Discrete Gaussian:}
The granularity of statistics released by SafeTab depends on the thresholds used as well as the noise scale used in Step 1 of the adaptive part of the algorithm. Under the MOE settings in Table~\ref{tab:moe-targets} the noise scales for Step 1 should be roughly the same under both SafeTab[Geometric] and SafeTab[Discrete Gaussian]. So we should expect statistics to be released at roughly the same granularity. A quantitative analysis requires running these algorithms on either the simulated or 2010 data, which we defer to future work. 

\paragraph{Alternate MOEs for Nation and State Detailed counts:}
It is evident from Table~\ref{tab:moe-targets} that most of the privacy loss results from releasing detailed counts for Nation and State population groups. We present in Table~\ref{tab:alternate-moes} the overall privacy loss that might result from changing the MOE slightly for (Nation, detailed) and (State, detailed) population group levels from 6 to 5, 7, 8, 9, 10 and 11. We did not increase beyond 11, as that is the MOE for County and AIANNH detailed population groups. We note that  increasing the MOE has a significant impact on the privacy loss. The zCDP (experimental) privacy loss bounds drops from around 12 to around 8, about a third reduction in the privacy loss.
